Simulation of parametrized cardiac electrophysiology in three dimensions using physics-informed neural networks

Physics-informed neural networks (PINNs) are extensively used to represent various physical systems across multiple scientific domains. The same can be said for cardiac electrophysiology, wherein fully-connected neural networks (FCNNs) have been employed to predict the evolution of an action potential in a 2D space following the two-parameter phenomenological Aliev-Panfilov (AP) model. In this paper, the training behaviour of PINNs is investigated to determine optimal hyperparameters to predict the electrophysiological activity of the myocardium in 3D according to the AP model, with the inclusion of boundary and material parameters. An FCNN architecture is employed with the governing partial differential equations in their strong form, which are scaled consistently with normalization of network inputs. The finite element (FE) method is used to generate training data for the network. Numerical examples with varying spatial dimensions and parameterizations are generated using the trained models. The network predicted fields for both the action potential and the recovery variable are compared with the respective FE simulations. Network losses are weighed with individual scalar values. Their effect on training and prediction is studied to arrive at a method of controlling losses during training.

==> figures/sec2/Graphs/fig.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=10.0cm]{figures/sec2/Graphs/alipan.eps}
    \caption{Illustration of the evolution of the non-dimensional action potential $\phi$ and the internal variable $r$ along the dimensionless time $\tau$ from a cellular perspective. The plot is generated using solutions to the AP equations obtained via the Newton algorithm.}
    \label{Fig:Ali_cell}
\end{figure}

==> figures/sec4/Diagrams/fig.tex <==
\begin{figure}[h]
    \centering
        \includegraphics[width=14.0cm]{figures/sec4/Diagrams/PINN_3d_EP_full.eps}
        \caption{Schematic diagram representing the architecture of the PINN trained for predicting cardiac electrophysiology in 3D. The network maps the normalized inputs $[\Bar{x},\;\Bar{y},\;\Bar{z},\;\Bar{t}]^\top$ to the predicted field $[\hat{\phi},\hat{r}]^\top$. PDE residuals $R_1,\;R_2$ and boundary residuals $\text{BC}_1,\;\text{BC}_2, \ldots$ etc. are linearly combined to get the final loss $\mathcal{L}$.}
        \label{Fig:PINN_scheme}
\end{figure}

==> figures/sec5/ex1-Loss-cont/fig.tex <==
\begin{figure}[ht]
    \begin{subfigure}[b]{.5\textwidth}
		\centering
			\includegraphics[width=7.0cm]{figures/sec5/ex1-Loss-cont/loss_no_clip1.eps}
			\caption{}
			\label{Fig:Loss_wo_clip}
    \end{subfigure}
    \begin{subfigure}[b]{.5\textwidth}
		\centering
			\includegraphics[width=7.0cm]{figures/sec5/ex1-Loss-cont/loss_clip1.eps}
			\caption{}
			\label{Fig:Loss_with_clip}
    \end{subfigure}
    \caption{Comparison of the effect of gradient clipping on training loss in Example 1. In contrast to the case $\textbf{(a)}$ without clipping, a significant reduction in gradient explosions is seen $\textbf{(b)}$ with gradient clipping.}
    \label{Fig:Loss_comp}
\end{figure}

==> figures/sec5/ex1-Loss-stim/fig.tex <==
\begin{figure}
    \begin{subfigure}[b]{.5\textwidth}
		\centering
			\includegraphics[width=7.0cm]{figures/sec5/ex1-Loss-stim/stim.eps}
			\caption{}
			\label{Fig:LossDiscont}
    \end{subfigure}
    \begin{subfigure}[b]{.5\textwidth}
		\centering
			\includegraphics[width=7.0cm]{figures/sec5/ex1-Loss-stim/loss_no_clip_discont.eps}
			\caption{}
			\label{Fig:Stim_ex1}
    \end{subfigure}
    \caption{Plot of exponential function approximation of external stimuli $I$ $[-]$ $\textbf{({a})}$ producing a training loss plot, $\textbf{(b)}$ for the discontinuous solution of Example 1.}
    \label{Fig:LossStim_discont}
\end{figure}

==> figures/sec5/ex1-cont/fig.tex <==
\begin{figure}

\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{c|c|c}

     765 GT Points [No clipping] & 5100 GT Points [No clipping] & 153 GT Points [With clipping]\\
     \includegraphics[width=4.8cm]{figures/sec5/ex1-cont/GT_points_1_5.eps} & \includegraphics[width=4.8cm]{figures/sec5/ex1-cont/GT_points_10.eps} & \includegraphics[width=4.8cm]{figures/sec5/ex1-cont/GT_points_3clip.eps}\\
    \hline
    \multicolumn{3}{c}{$c=4$ $[-]$}\\
    \hline
     \includegraphics[width=4.8cm]{figures/sec5/ex1-cont/comp_1_5_c4.eps} & \includegraphics[width=4.8cm]{figures/sec5/ex1-cont/comp_10_c4.eps} & \includegraphics[width=4.8cm]{figures/sec5/ex1-cont/comp_3clip_c4.eps}\\
    \hline
    \multicolumn{3}{c}{$c=6$ $[-]$}\\
    \hline
     \includegraphics[width=4.8cm]{figures/sec5/ex1-cont/comp_1_5_c6.eps} & \includegraphics[width=4.8cm]{figures/sec5/ex1-cont/comp_10_c6.eps} & \includegraphics[width=4.8cm]{figures/sec5/ex1-cont/comp_3clip_c6.eps}\\
    \hline
    \multicolumn{3}{c}{$c=8$ $[-]$}\\
    \hline
     \includegraphics[width=4.8cm]{figures/sec5/ex1-cont/comp_1_5_c8.eps} & \includegraphics[width=4.8cm]{figures/sec5/ex1-cont/comp_10_c8.eps} & \includegraphics[width=4.8cm]{figures/sec5/ex1-cont/comp_3clip_c8.eps}\\
    \hline
     \multicolumn{3}{c}{\includegraphics[width=8.0cm]{figures/sec5/ex1-cont/legend1.eps}}\\
    \hline
\end{tabular}
\renewcommand{\arraystretch}{1}
\caption{Study of the effect of gradient clipping on the PINN prediction of the solution to the AP equations. The plots compare the predicted variables $\hat{\phi}$ and $\hat{r}$ against ground truth (GT) values $\phi$ and $r$ for different values of material parameter $c$ which changes column-wise.}
\label{Fig:Result_ex1_cont}
\end{figure}

==> figures/sec5/ex1-discont/fig.tex <==
\begin{figure}
    \begin{subfigure}{\linewidth}
        \centering
        \renewcommand{\arraystretch}{1.2}
        \begin{tabular}{c|c|c}
            \hline
             $c=4$ $[-]$ & $c=6$ $[-]$ & $c=8$ $[-]$\\
            \hline
            \multicolumn{3}{c}{$\alpha_1=10^{-4},\;\alpha_2=10^{-2},\;\alpha_{\text{GT}}=1$}\\
            \hline
             \includegraphics[width=4.8cm]{figures/sec5/ex1-discont/comp_6clip_c4.eps} & \includegraphics[width=4.8cm]{figures/sec5/ex1-discont/comp_6clip_c6.eps} & \includegraphics[width=4.8cm]{figures/sec5/ex1-discont/comp_6clip_c8.eps}\\
            \hline
            \multicolumn{3}{c}{$\alpha_1=10^{-3},\;\alpha_2=10^{-2},\;\alpha_{\text{GT}}=1$}\\
            \hline
             \includegraphics[width=4.8cm]{figures/sec5/ex1-discont/comp_11clip_c4.eps} & \includegraphics[width=4.8cm]{figures/sec5/ex1-discont/comp_11clip_c6.eps} & \includegraphics[width=4.8cm]{figures/sec5/ex1-discont/comp_11clip_c8.eps}\\
            \hline
             \multicolumn{3}{c}{\includegraphics[width=8.0cm]{figures/sec5/ex1-cont/legend1.eps}}\\
            \hline
        \end{tabular}
        \renewcommand{\arraystretch}{1}
        \caption{}
        \label{Fig:Result_ex1_discont_c}
    \end{subfigure}

    \begin{subfigure}{\linewidth}
        \centering
        \renewcommand{\arraystretch}{1.2}
        \begin{tabular}{c|c|c}
            \hline
             $\Bar{\tau}_\text{stim}=20$ $\text{ms}$ & $\Bar{\tau}_\text{stim}=40 $ $\text{ms}$ & $\Bar{\tau}_\text{stim}=60$ $\text{ms}$\\
            \hline
            \multicolumn{3}{c}{$\alpha_1=10^{-3},\;\alpha_2=10^{-2},\;\alpha_{\text{GT}}=1$}\\
            \hline
             \includegraphics[width=4.8cm]{figures/sec5/ex1-discont/comp_2clip_c20.eps} & \includegraphics[width=4.8cm]{figures/sec5/ex1-discont/comp_2clip_c44.eps} & \includegraphics[width=4.8cm]{figures/sec5/ex1-discont/comp_2clip_c60.eps}\\
            \hline
             \multicolumn{3}{c}{\includegraphics[width=8.0cm]{figures/sec5/ex1-cont/legend1.eps}}\\
            \hline
        \end{tabular}
        \renewcommand{\arraystretch}{1}
        \caption{}
        \label{Fig:Result_ex1_timepara}
    \end{subfigure}
    \caption{Study of the effect of loss weights $\alpha_i$ on the PINN prediction of the solution to the AP equations. The plots compare the predicted variables $\hat{\phi}$ and $\hat{r}$ against ground truth (GT) values $\phi$ and $r$. $\textbf{(a)}$ The material parameter $\Bar{c}$ is parametrized while $\textbf{(b)}$ the timing of application of external stimuli $\Bar{\tau}_\text{stim}$ is parametrized.}
    \label{Fig:Result_ex1_discont}
\end{figure}

==> figures/sec5/ex2-Graphs/fig.tex <==
\begin{figure}[h!]
    \centering
        \includegraphics[width=16cm]{figures/sec5/ex2-Graphs/Loss_weights.eps}
    \caption{Semi-log plot of MSE loss $\text{BC}_\text{GT}$ between predicted action potential $\hat{\Phi}$ and FEM generated GT points $\Phi$ for trials 1 and 2 during training. Right axis marks the loss weight $\alpha_1$ for loss $R_1$, which is controlled during training according to \autoref{Eq:stg_loss_wt}.}
    \label{Fig:Staged_loss_wt}
\end{figure}

==> figures/sec5/ex2-SampleStudy/fig.tex <==
\begin{figure}[h!]
    \centering
        \includegraphics[width=10cm]{figures/sec5/ex2-SampleStudy/sample_study.eps}
    \caption{Sensitivity analysis of the prediction error of the PINN (RMSE $\Phi$) with respect to the number of GT points (interior) included during training for Example 2, trial 2.}
    \label{Fig:Sample_study}
\end{figure}

==> figures/sec5/ex2-T22/fig.tex <==
\begin{figure}

\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{>{\centering}m{2.725cm}>{\centering}m{2.725cm}>{\centering}m{2.725cm}>{\centering}m{2.7cm}c}
            % {|>{\centering}m{0.17\textwidth}|>{\centering}m{0.145\textwidth}|>{\centering}m{0.175\textwidth}|>{\centering}m{0.1\textwidth}|c|}
    \hline
     $\hat{\Phi}\;[\text{mV}]$ & $\Phi\;[\text{mV}]$ & Absolute error [mV] & $\hat{r}\;[-]$ & $r\;[-]$\\
    \hline
     \multicolumn{5}{c}{\includegraphics[width=16cm]{figures/sec5/ex2-T22/T22_40s.eps}}\\
    \hline
    \multicolumn{5}{c}{$t=40\;[\text{ms}]$}\\
    \hline
     \multicolumn{5}{c}{\includegraphics[width=16cm]{figures/sec5/ex2-T22/T22_490s.eps}}\\
    \hline
    \multicolumn{5}{c}{$t=490\;[\text{ms}]$}\\
    \hline
     \multicolumn{5}{c}{\includegraphics[width=16cm]{figures/sec5/ex2-T22/T22_540s.eps}}\\
    \hline
    \multicolumn{5}{c}{$t=540\;[\text{ms}]$}\\
    \hline
     \multicolumn{5}{c}{\includegraphics[width=16cm]{figures/sec5/ex2-T22/T22_650s.eps}}\\
    \hline
    \multicolumn{5}{c}{$t=650\;[\text{ms}]$}\\
    \hline
    \multicolumn{5}{c}{\includegraphics[width=16cm]{figures/sec5/ex2-T35/Legend_2.eps}}\\
    \hline
\end{tabular}
\renewcommand{\arraystretch}{1}
\caption{Results from Example 2, trial 1. Column 1 and 4: 3D contour plots of predictions of output variables $\hat{\Phi}$, $\hat{r}$ by a PINN trained with loss weights. Column 2 and 5: FEM generated GT values $\Phi$, $r$. Column 3: Absolute error $\epsilon_\Phi$ between $\hat{\Phi}$ and $\Phi$ at different time stamps for the generation of a scroll wave.}
\label{Fig:Result_ex2_T22}
\end{figure}

==> figures/sec5/ex2-T35/fig.tex <==
\begin{figure}

\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{{>{\centering}m{2.725cm}>{\centering}m{2.725cm}>{\centering}m{2.725cm}>{\centering}m{2.7cm}c}}
    \hline
     $\hat{\Phi}\;[\text{mV}]$ & $\Phi\;[\text{mV}]$ & Absolute error [mV] & $\hat{r}\;[-]$ & $r\;[-]$\\
    \hline
     \multicolumn{5}{c}{\includegraphics[width=16cm]{figures/sec5/ex2-T35/T35_40s.eps}}\\
    \hline
    \multicolumn{5}{c}{$t=40\;[\text{ms}]$}\\
    \hline
     \multicolumn{5}{c}{\includegraphics[width=16cm]{figures/sec5/ex2-T35/T35_490s.eps}}\\
    \hline
    \multicolumn{5}{c}{$t=490\;[\text{ms}]$}\\
    \hline
     \multicolumn{5}{c}{\includegraphics[width=16cm]{figures/sec5/ex2-T35/T35_540s.eps}}\\
    \hline
    \multicolumn{5}{c}{$t=540\;[\text{ms}]$}\\
    \hline
     \multicolumn{5}{c}{\includegraphics[width=16cm]{figures/sec5/ex2-T35/T35_650s.eps}}\\
    \hline
    \multicolumn{5}{c}{$t=650\;[\text{ms}]$}\\
    \hline
     \multicolumn{5}{c}{\includegraphics[width=16cm]{figures/sec5/ex2-T35/Legend_2.eps}}\\
    \hline
\end{tabular}
\renewcommand{\arraystretch}{1}
\caption{Results from Example 2, trial 2. Column 1 and 4: 3D contour plots of predictions of output variables $\hat{\Phi}$, $\hat{r}$ by a PINN trained with a staged reduction of loss weights. Column 2 and 5: FEM generated GT values $\Phi$, $r$. Column 3: Absolute error $\epsilon_\Phi$ between $\hat{\Phi}$ and $\Phi$ at different time stamps for the generation of a scroll wave.}
\label{Fig:Result_ex2_T35}
\end{figure}

==> figures/sec5/ex3/fig.tex <==
\begin{figure}
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{{>{\centering}m{2.725cm}>{\centering}m{2.725cm}>{\centering}m{2.725cm}>{\centering}m{2.7cm}c}}
    \hline
     $t=40\;[\text{ms}]$ & $t=480\;[\text{ms}]$ & $t=580\;[\text{ms}]$ & $t=740\;[\text{ms}]$ & $t=1850\;[\text{ms}]$\\
    \hline
     \multicolumn{5}{c}{\includegraphics[width=16cm]{figures/sec5/ex3/phi_tst_420.eps}}\\
    \hline
    \multicolumn{5}{c}{$t_\text{stim}=430\;[\text{ms}]$}\\
    \hline
     \multicolumn{5}{c}{\includegraphics[width=16cm]{figures/sec5/ex3/phi_tst_440.eps}}\\
    \hline
    \multicolumn{5}{c}{$t_\text{stim}=450\;[\text{ms}]$}\\
    \hline
     \multicolumn{5}{c}{\includegraphics[width=16cm]{figures/sec5/ex3/phi_tst_470.eps}}\\
    \hline
    \multicolumn{5}{c}{$t_\text{stim}=480\;[\text{ms}]$}\\
    \hline
     \multicolumn{5}{c}{\includegraphics[width=16cm]{figures/sec5/ex3/Legend_3.eps}}\\
    \hline
\end{tabular}
\renewcommand{\arraystretch}{1}
\caption{3D contour plots of action potential $\hat{\Phi}$ at different time steps generated by a PINN trained with $\Bar{t}_\text{stim}$ as an additional input. A sustained scroll wave is seen only for $t_\text{stim}=480\;\text{ms}$.}
\label{Fig:Result_ex3}
\end{figure}
